Scalable Cross Validation Losses for Gaussian Process Models

We introduce a simple and scalable method for training Gaussian process (GP) models that exploits cross-validation and nearest neighbor truncation. To accommodate binary and multi-class classification we leverage P\`olya-Gamma auxiliary variables and variational inference. In an extensive empirical comparison with a number of alternative methods for scalable GP regression and classification, we find that our method offers fast training and excellent predictive performance. We argue that the good predictive performance can be traced to the non-parametric nature of the resulting predictive distributions as well as to the cross-validation loss, which provides robustness against model mis-specification.

==> binary_class_ranks.tex <==
\begin{tabular}{ccccc}
\toprule
{} &   &               SVGP &               PGVI & LOO-$k$ \\
Value &           &                    &                    &         \\
\midrule
NLL   &   &  $\mathbf{ 1.89 }$ &             $2.04$ &  $2.07$ \\
Error &   &             $1.99$ &  $\mathbf{ 1.88 }$ &  $2.13$ \\
\bottomrule
\end{tabular}


==> binary_classification_full.tex <==
\begin{tabular}{ccccccc}
\toprule
      &              &   &                          SVGP &                          PGVI &                       LOO-$k$ \\
Metric & Dataset &           &                               &                               &                               \\
\midrule
\midrule
NLL & Titanic &   &  $\mathbf{ 0.482 \pm 0.019 }$ &  $\mathbf{ 0.483 \pm 0.018 }$ &  $\mathbf{ 0.485 \pm 0.021 }$ \\
      & Bank &   &  $\mathbf{ 0.241 \pm 0.006 }$ &  $\mathbf{ 0.246 \pm 0.007 }$ &  $\mathbf{ 0.234 \pm 0.008 }$ \\
      & Spambase &   &  $\mathbf{ 0.213 \pm 0.004 }$ &  $\mathbf{ 0.217 \pm 0.002 }$ &             $0.222 \pm 0.003$ \\
      & Musk-2 &   &             $0.126 \pm 0.003$ &  $\mathbf{ 0.114 \pm 0.003 }$ &  $\mathbf{ 0.111 \pm 0.005 }$ \\
      & Adult &   &  $\mathbf{ 0.309 \pm 0.002 }$ &             $0.319 \pm 0.002$ &             $0.329 \pm 0.002$ \\
      & Higgs &   &  $\mathbf{ 0.617 \pm 0.002 }$ &  $\mathbf{ 0.619 \pm 0.002 }$ &             $0.629 \pm 0.001$ \\
      & Susy &   &  $\mathbf{ 0.440 \pm 0.001 }$ &  $\mathbf{ 0.442 \pm 0.002 }$ &             $0.468 \pm 0.002$ \\
      & Covtype-Fir &   &             $0.377 \pm 0.001$ &             $0.354 \pm 0.000$ &  $\mathbf{ 0.057 \pm 0.001 }$ \\
      & Covtype-Pine &   &             $0.381 \pm 0.001$ &             $0.357 \pm 0.001$ &  $\mathbf{ 0.060 \pm 0.001 }$ \\
Error & Titanic &   &  $\mathbf{ 0.210 \pm 0.011 }$ &  $\mathbf{ 0.209 \pm 0.011 }$ &  $\mathbf{ 0.210 \pm 0.011 }$ \\
      & Bank &   &  $\mathbf{ 0.098 \pm 0.004 }$ &  $\mathbf{ 0.102 \pm 0.004 }$ &  $\mathbf{ 0.101 \pm 0.006 }$ \\
      & Spambase &   &  $\mathbf{ 0.067 \pm 0.002 }$ &  $\mathbf{ 0.066 \pm 0.002 }$ &             $0.076 \pm 0.003$ \\
      & Musk-2 &   &             $0.036 \pm 0.001$ &  $\mathbf{ 0.033 \pm 0.001 }$ &  $\mathbf{ 0.034 \pm 0.002 }$ \\
      & Adult &   &  $\mathbf{ 0.142 \pm 0.001 }$ &             $0.147 \pm 0.002$ &             $0.146 \pm 0.001$ \\
      & Higgs &   &  $\mathbf{ 0.340 \pm 0.002 }$ &  $\mathbf{ 0.341 \pm 0.002 }$ &             $0.348 \pm 0.001$ \\
      & Susy &   &  $\mathbf{ 0.202 \pm 0.001 }$ &  $\mathbf{ 0.205 \pm 0.001 }$ &             $0.219 \pm 0.001$ \\
      & Covtype-Fir &   &             $0.171 \pm 0.000$ &             $0.161 \pm 0.001$ &  $\mathbf{ 0.023 \pm 0.000 }$ \\
      & Covtype-Pine &   &             $0.174 \pm 0.001$ &             $0.163 \pm 0.001$ &  $\mathbf{ 0.024 \pm 0.000 }$ \\
\bottomrule
\end{tabular}


==> degenerate.tex <==
\begin{table}
  \centering
  \caption{
      \hspace{-1.10em}
    We summarize the results for the experiment in Sec.~\ref{sec:degenerate} exploring
    the performance of LOO-64 and SVGP-512 on degenerate datasets. We report both test log likelihood and
    RMSE on held out test data.}
    \label{table:degnerate}
  \resizebox{0.8\linewidth}{!}{%
\begin{tabular}{cc|cc|ccccc}
\toprule
    {} &   &    {\bf Original} &      & {\bf Degenerate} &       &  \\
    {\bf Dataset} & {\bf Method}  &    Log Likelihood   & RMSE & Log Likelihood     &  RMSE &  \\
\midrule
Bike   & SVGP-512   &  $0.859$     &  $0.082$ &  $0.553$ &  $0.118$ &    \\
Bike  & LOO-64 &  $2.498$     &  $0.50$ &  $-0.912$ &  $0.224$ &  \\ 
Elevators   & SVGP-512   &  $-1.111$     &  $0.505$ &  $-1.107$ &  $0.493$ &    \\
Elevators  & LOO-64 &  $-0.414$     &  $0.369$ &  $-3.783$ &  $0.676$ &  \\ 
Pol   & SVGP-512   &  $-1.040$     &  $0.367$ &  $-1.054$ &  $0.393$ &    \\
Pol  & LOO-64 &  $1.162$     &  $0.077$ &  $0.689$ &  $0.128$ &  \\ 
Slice   & SVGP-512   &  $0.611$     &  $0.110$ &  $0.726$ &  $0.099$ &    \\
Slice& LOO-64 &  $2.723$     &  $0.023$ &  $2.787$ &  $0.023$ &  \\ 
\bottomrule
\end{tabular}
  }
    \label{table:degenerate}
\end{table}
%%%

%Dataset	Method	No degeneracy added	With degeneracy
%bike	SVGP-512	0.859 / 0.082	0.553 / 0.118
%bike	LOO-64	2.498 / 0.050	-0.912 / 0.224
%elevators	SVGP-512	-1.111 / 0.505	-1.107 / 0.493
%elevators	LOO-64	-0.414 / 0.369	-3.783 / 0.676
%pol	SVGP-512	-1.040 / 0.367	-1.054 / 0.393
%pol	LOO-64	1.162 / 0.077	0.689 / 0.128
%slice	SVGP-512	0.611 / 0.110	0.726 / 0.099
%slice	LOO-64	2.723 / 0.023	2.787 / 0.023


==> multi_class_ranks.tex <==
\begin{tabular}{cccc}
\toprule
{} &   &    SVGP &            LOO-$k$ \\
Value &           &         &                    \\
\midrule
NLL   &   &  $1.63$ &  $\mathbf{ 1.37 }$ \\
Error &   &  $1.68$ &  $\mathbf{ 1.32 }$ \\
\bottomrule
\end{tabular}


==> multi_classification_full.tex <==
\begin{tabular}{cccccc}
\toprule
      &         &   &                          SVGP &                       LOO-$k$ \\
Metric & Dataset &           &                               &                               \\
\midrule
\midrule
NLL & Cardio &   &  $\mathbf{ 0.387 \pm 0.018 }$ &             $0.466 \pm 0.020$ \\
      & Molec &   &             $0.030 \pm 0.004$ &  $\mathbf{ 0.025 \pm 0.001 }$ \\
      & Abalone &   &  $\mathbf{ 0.691 \pm 0.013 }$ &  $\mathbf{ 0.668 \pm 0.018 }$ \\
      & Wine &   &             $0.996 \pm 0.009$ &  $\mathbf{ 0.945 \pm 0.008 }$ \\
      & Page &   &  $\mathbf{ 0.147 \pm 0.010 }$ &  $\mathbf{ 0.129 \pm 0.010 }$ \\
      & Optical &   &  $\mathbf{ 0.080 \pm 0.005 }$ &             $0.098 \pm 0.004$ \\
      & Landsat &   &  $\mathbf{ 0.197 \pm 0.009 }$ &  $\mathbf{ 0.199 \pm 0.011 }$ \\
      & Thyroid &   &             $0.099 \pm 0.007$ &  $\mathbf{ 0.068 \pm 0.006 }$ \\
      & Pendigits &   &  $\mathbf{ 0.026 \pm 0.004 }$ &  $\mathbf{ 0.032 \pm 0.003 }$ \\
      & Nursery &   &  $\mathbf{ 0.033 \pm 0.001 }$ &  $\mathbf{ 0.033 \pm 0.001 }$ \\
      & Chess &   &  $\mathbf{ 0.034 \pm 0.005 }$ &  $\mathbf{ 0.031 \pm 0.002 }$ \\
      & Shuttle &   &             $0.015 \pm 0.001$ &  $\mathbf{ 0.010 \pm 0.000 }$ \\
      & Covtype &   &             $0.560 \pm 0.002$ &  $\mathbf{ 0.089 \pm 0.001 }$ \\
\midrule
Error & Cardio &   &  $\mathbf{ 0.146 \pm 0.007 }$ &             $0.168 \pm 0.006$ \\
      & Molec &   &  $\mathbf{ 0.001 \pm 0.001 }$ &  $\mathbf{ 0.000 \pm 0.000 }$ \\
      & Abalone &   &             $0.314 \pm 0.008$ &  $\mathbf{ 0.289 \pm 0.008 }$ \\
      & Wine &   &             $0.414 \pm 0.008$ &  $\mathbf{ 0.355 \pm 0.009 }$ \\
      & Page &   &             $0.045 \pm 0.003$ &  $\mathbf{ 0.035 \pm 0.003 }$ \\
      & Optical &   &             $0.020 \pm 0.002$ &  $\mathbf{ 0.014 \pm 0.002 }$ \\
      & Landsat &   &  $\mathbf{ 0.078 \pm 0.005 }$ &  $\mathbf{ 0.075 \pm 0.005 }$ \\
      & Thyroid &   &             $0.044 \pm 0.003$ &  $\mathbf{ 0.019 \pm 0.002 }$ \\
      & Pendigits &   &  $\mathbf{ 0.005 \pm 0.000 }$ &             $0.006 \pm 0.001$ \\
      & Nursery &   &  $\mathbf{ 0.008 \pm 0.001 }$ &             $0.010 \pm 0.001$ \\
      & Chess &   &  $\mathbf{ 0.009 \pm 0.001 }$ &  $\mathbf{ 0.009 \pm 0.001 }$ \\
      & Shuttle &   &             $0.005 \pm 0.001$ &  $\mathbf{ 0.002 \pm 0.000 }$ \\
      & Covtype &   &             $0.238 \pm 0.001$ &  $\mathbf{ 0.032 \pm 0.000 }$ \\
\bottomrule
\end{tabular}


==> multi_regression_full.tex <==
\begin{tabular}{cccccccc}
\toprule
     &        &   &                          SVGP &               PPGPR &                        MLL-$k$ &                        LOO-$k$ \\
Metric & Dataset &           &                               &                     &                                &                                \\
\midrule
\midrule
NLL & Rt.-Baxter &   &            $-0.003 \pm 0.008$ &  $-0.087 \pm 0.001$ &  $\mathbf{ -1.123 \pm 0.004 }$ &             $-0.911 \pm 0.006$ \\
     & Fw.-Baxter &   &            $-1.353 \pm 0.001$ &  $-1.717 \pm 0.001$ &             $-1.936 \pm 0.001$ &  $\mathbf{ -1.961 \pm 0.000 }$ \\
     & Fw.-Kuka &   &            $-1.060 \pm 0.001$ &  $-1.557 \pm 0.001$ &  $\mathbf{ -1.892 \pm 0.003 }$ &  $\mathbf{ -1.886 \pm 0.003 }$ \\
     & Sarcos &   &            $-0.862 \pm 0.000$ &  $-1.095 \pm 0.001$ &             $-1.439 \pm 0.003$ &  $\mathbf{ -1.473 \pm 0.003 }$ \\
RMSE & Rt.-Baxter &   &             $0.583 \pm 0.015$ &   $0.609 \pm 0.028$ &   $\mathbf{ 0.106 \pm 0.001 }$ &              $0.152 \pm 0.002$ \\
     & Fw.-Baxter &   &             $0.043 \pm 0.000$ &   $0.053 \pm 0.001$ &   $\mathbf{ 0.035 \pm 0.000 }$ &              $0.036 \pm 0.000$ \\
     & Fw.-Kuka &   &  $\mathbf{ 0.089 \pm 0.000 }$ &   $0.093 \pm 0.000$ &              $0.115 \pm 0.001$ &              $0.115 \pm 0.001$ \\
     & Sarcos &   &             $0.105 \pm 0.000$ &   $0.110 \pm 0.000$ &   $\mathbf{ 0.076 \pm 0.001 }$ &              $0.077 \pm 0.001$ \\
\bottomrule
\end{tabular}


==> multi_regression_ranks.tex <==
\begin{tabular}{cccccc}
\toprule
{} &   &    SVGP &   PPGPR &            MLL-$k$ &            LOO-$k$ \\
Value &           &         &         &                    &                    \\
\midrule
NLL   &   &  $3.94$ &  $3.06$ &             $1.57$ &  $\mathbf{ 1.43 }$ \\
RMSE  &   &  $2.61$ &  $3.39$ &  $\mathbf{ 1.80 }$ &             $2.20$ \\
\bottomrule
\end{tabular}


==> tables/uci_ranks.tex <==
\begin{tabular}{ccccccccc}
\toprule
{} &   &    SVGP &   PPGPR & Vecchia &     ALC & MLL-$k$ &                LOO-$k$ \\
\midrule
NLL   &   &  $4.20$     &  $2.33$ &  $4.86$ &  $3.94$ &    $2.41$ &  $\mathbf{ 2.02 }$ \\
RMSE  &   &  $3.01$     &  $4.99$ &  $4.16$ &  $4.17$ &    $2.33$ &  $\mathbf{ 2.14 }$ \\
CRPS &   &  $4.43$      &  $2.61$ &  $5.15$ &  $3.27$ &    $2.55$ &  $\mathbf{ 2.05 }$ \\
\bottomrule
\end{tabular}


==> uci_ranks.tex <==
\begin{tabular}{ccccccccc}
\toprule
{} &   &    SVGP &   PPGPR & Vecchia &     ALC & MLL-$k$ &                LOO-$k$ \\
\midrule
NLL   &   &  $4.20$     &  $2.33$ &  $4.86$ &  $3.94$ &    $2.41$ &  $\mathbf{ 2.02 }$ \\
RMSE  &   &  $3.01$     &  $4.99$ &  $4.16$ &  $4.17$ &    $2.33$ &  $\mathbf{ 2.14 }$ \\
CRPS &   &  $4.43$      &  $2.61$ &  $5.15$ &  $3.27$ &    $2.55$ &  $\mathbf{ 2.05 }$ \\
\bottomrule
\end{tabular}


==> univariate_regression_full.tex <==
\begin{tabular}{cccccccccccc}
\toprule
     &            &   &                           MLL &                          SVGP &                          PPGPR &                       Vecchia &               SWSGP &                            ALC &                       MLL-$k$ &                        LOO-$k$ \\
Metric & Dataset &           &                               &                               &                                &                               &                     &                                &                               &                                \\
\midrule
\midrule
NLL & Pol &   &            $-0.817 \pm 0.001$ &            $-0.651 \pm 0.005$ &             $-0.825 \pm 0.005$ &            $-1.190 \pm 0.015$ &  $-1.036 \pm 0.022$ &  $\mathbf{ -1.696 \pm 0.012 }$ &            $-1.200 \pm 0.014$ &             $-1.238 \pm 0.018$ \\
     & Elevators &   &             $0.398 \pm 0.013$ &             $0.401 \pm 0.007$ &   $\mathbf{ 0.329 \pm 0.007 }$ &             $0.407 \pm 0.007$ &   $0.651 \pm 0.015$ &              $0.441 \pm 0.012$ &             $0.397 \pm 0.007$ &              $0.401 \pm 0.008$ \\
     & Bike &   &            $-1.750 \pm 0.014$ &            $-0.807 \pm 0.007$ &             $-1.314 \pm 0.007$ &            $-1.743 \pm 0.053$ &  $-1.401 \pm 0.020$ &             $-1.397 \pm 0.013$ &            $-2.541 \pm 0.008$ &  $\mathbf{ -2.771 \pm 0.031 }$ \\
     & Kin40K &   &            $-0.075 \pm 0.001$ &            $-0.414 \pm 0.002$ &             $-0.770 \pm 0.002$ &            $-0.763 \pm 0.002$ &  $-0.694 \pm 0.008$ &             $-0.778 \pm 0.003$ &            $-0.884 \pm 0.002$ &  $\mathbf{ -1.040 \pm 0.030 }$ \\
     & Protein &   &             $0.875 \pm 0.002$ &             $0.902 \pm 0.003$ &              $0.747 \pm 0.008$ &             $0.936 \pm 0.011$ &   $0.804 \pm 0.006$ &              $0.826 \pm 0.020$ &  $\mathbf{ 0.635 \pm 0.007 }$ &   $\mathbf{ 0.626 \pm 0.008 }$ \\
     & Keggdir. &   &            $-0.870 \pm 0.052$ &            $-1.045 \pm 0.017$ &  $\mathbf{ -1.601 \pm 0.016 }$ &            $-1.048 \pm 0.016$ &  $-1.033 \pm 0.019$ &                            --- &            $-1.055 \pm 0.019$ &             $-1.068 \pm 0.015$ \\
     & Slice &   &            $-1.240 \pm 0.004$ &            $-1.267 \pm 0.003$ &             $-1.516 \pm 0.004$ &            $-1.648 \pm 0.007$ &  $-1.797 \pm 0.016$ &             $-2.441 \pm 0.003$ &            $-2.572 \pm 0.002$ &  $\mathbf{ -2.753 \pm 0.027 }$ \\
     & Keggundir. &   &            $-0.643 \pm 0.008$ &            $-0.704 \pm 0.006$ &  $\mathbf{ -1.807 \pm 0.018 }$ &            $-0.696 \pm 0.004$ &  $-0.690 \pm 0.005$ &              $0.498 \pm 0.310$ &            $-0.697 \pm 0.005$ &             $-0.714 \pm 0.006$ \\
\midrule
RMSE & Pol &   &  $\mathbf{ 0.074 \pm 0.001 }$ &             $0.107 \pm 0.002$ &              $0.111 \pm 0.002$ &  $\mathbf{ 0.075 \pm 0.002 }$ &   $0.091 \pm 0.002$ &              $0.083 \pm 0.001$ &             $0.077 \pm 0.002$ &   $\mathbf{ 0.073 \pm 0.001 }$ \\
     & Elevators &   &  $\mathbf{ 0.347 \pm 0.007 }$ &             $0.360 \pm 0.003$ &              $0.362 \pm 0.003$ &             $0.362 \pm 0.003$ &   $0.448 \pm 0.004$ &              $0.376 \pm 0.003$ &             $0.359 \pm 0.003$ &              $0.360 \pm 0.003$ \\
     & Bike &   &  $\mathbf{ 0.022 \pm 0.001 }$ &             $0.088 \pm 0.002$ &              $0.094 \pm 0.002$ &             $0.029 \pm 0.002$ &   $0.059 \pm 0.002$ &              $0.098 \pm 0.002$ &  $\mathbf{ 0.025 \pm 0.002 }$ &              $0.028 \pm 0.002$ \\
     & Kin40K &   &  $\mathbf{ 0.084 \pm 0.005 }$ &             $0.147 \pm 0.001$ &              $0.188 \pm 0.002$ &             $0.117 \pm 0.000$ &   $0.121 \pm 0.001$ &              $0.129 \pm 0.001$ &             $0.105 \pm 0.000$ &              $0.095 \pm 0.003$ \\
     & Protein &   &  $\mathbf{ 0.514 \pm 0.003 }$ &             $0.594 \pm 0.002$ &              $0.609 \pm 0.002$ &             $0.595 \pm 0.007$ &   $0.542 \pm 0.003$ &              $0.571 \pm 0.002$ &             $0.525 \pm 0.002$ &              $0.526 \pm 0.003$ \\
     & Keggdir. &   &             $0.090 \pm 0.004$ &  $\mathbf{ 0.086 \pm 0.001 }$ &              $0.089 \pm 0.002$ &  $\mathbf{ 0.085 \pm 0.001 }$ &   $0.087 \pm 0.001$ &                            --- &  $\mathbf{ 0.085 \pm 0.001 }$ &   $\mathbf{ 0.084 \pm 0.001 }$ \\
     & Slice &   &             $0.031 \pm 0.003$ &             $0.051 \pm 0.001$ &              $0.095 \pm 0.001$ &             $0.038 \pm 0.002$ &   $0.041 \pm 0.001$ &              $0.026 \pm 0.002$ &  $\mathbf{ 0.021 \pm 0.001 }$ &              $0.024 \pm 0.001$ \\
     & Keggundir. &   &  $\mathbf{ 0.119 \pm 0.002 }$ &             $0.120 \pm 0.001$ &              $0.124 \pm 0.001$ &             $0.120 \pm 0.001$ &   $0.124 \pm 0.001$ &   $\mathbf{ 0.118 \pm 0.001 }$ &             $0.121 \pm 0.001$ &   $\mathbf{ 0.117 \pm 0.001 }$ \\
\midrule
CRPS & Pol &   &             $0.051 \pm 0.000$ &             $0.061 \pm 0.000$ &              $0.057 \pm 0.000$ &             $0.039 \pm 0.000$ &   $0.042 \pm 0.001$ &   $\mathbf{ 0.034 \pm 0.000 }$ &             $0.039 \pm 0.000$ &              $0.036 \pm 0.001$ \\
     & Elevators &   &  $\mathbf{ 0.195 \pm 0.003 }$ &             $0.198 \pm 0.001$ &   $\mathbf{ 0.193 \pm 0.001 }$ &             $0.199 \pm 0.001$ &   $0.244 \pm 0.002$ &              $0.205 \pm 0.002$ &             $0.197 \pm 0.001$ &              $0.197 \pm 0.001$ \\
     & Bike &   &             $0.019 \pm 0.000$ &             $0.049 \pm 0.000$ &              $0.037 \pm 0.000$ &             $0.018 \pm 0.001$ &   $0.026 \pm 0.000$ &              $0.040 \pm 0.000$ &             $0.009 \pm 0.000$ &   $\mathbf{ 0.008 \pm 0.000 }$ \\
     & Kin40K &   &             $0.093 \pm 0.000$ &             $0.082 \pm 0.000$ &              $0.077 \pm 0.000$ &             $0.063 \pm 0.000$ &   $0.063 \pm 0.000$ &              $0.066 \pm 0.000$ &             $0.054 \pm 0.000$ &   $\mathbf{ 0.047 \pm 0.001 }$ \\
     & Protein &   &             $0.293 \pm 0.001$ &             $0.326 \pm 0.001$ &              $0.310 \pm 0.001$ &             $0.333 \pm 0.004$ &   $0.285 \pm 0.001$ &              $0.285 \pm 0.001$ &  $\mathbf{ 0.259 \pm 0.001 }$ &   $\mathbf{ 0.260 \pm 0.001 }$ \\
     & Keggdir. &   &             $0.046 \pm 0.002$ &             $0.037 \pm 0.000$ &   $\mathbf{ 0.031 \pm 0.000 }$ &             $0.038 \pm 0.000$ &   $0.038 \pm 0.000$ &                            --- &             $0.037 \pm 0.001$ &              $0.035 \pm 0.000$ \\
     & Slice &   &             $0.029 \pm 0.000$ &             $0.031 \pm 0.000$ &              $0.032 \pm 0.000$ &             $0.022 \pm 0.000$ &   $0.019 \pm 0.000$ &              $0.012 \pm 0.000$ &             $0.009 \pm 0.000$ &   $\mathbf{ 0.009 \pm 0.000 }$ \\
     & Keggundir. &   &             $0.056 \pm 0.001$ &             $0.051 \pm 0.000$ &              $0.036 \pm 0.000$ &             $0.053 \pm 0.000$ &   $0.052 \pm 0.000$ &   $\mathbf{ 0.033 \pm 0.000 }$ &             $0.051 \pm 0.000$ &              $0.050 \pm 0.000$ \\
\bottomrule
\end{tabular}


==> univariate_regression_ranks.tex <==
\begin{tabular}{ccccccccc}
\toprule
{} &   &    SVGP &   PPGPR & Vecchia &   SWSGP &     ALC & MLL-$k$ &            LOO-$k$ \\
Value &           &         &         &         &         &         &         &                    \\
\midrule
NLL   &   &  $5.60$ &  $3.51$ &  $4.64$ &  $5.16$ &  $4.41$ &  $2.64$ &  $\mathbf{ 2.04 }$ \\
RMSE  &   &  $4.59$ &  $6.21$ &  $3.44$ &  $4.76$ &  $4.67$ &  $2.34$ &  $\mathbf{ 1.99 }$ \\
CRPS  &   &  $5.78$ &  $4.09$ &  $4.69$ &  $4.74$ &  $4.06$ &  $2.65$ &  $\mathbf{ 2.00 }$ \\
\bottomrule
\end{tabular}

